SPAMming Labels: Efficient Annotations for the Trackers of Tomorrow

Increasing the annotation efficiency of trajectory annotations from videos has the potential to enable the next generation of data-hungry tracking algorithms to thrive on large-scale datasets. Despite the importance of this task, there are currently very few works exploring how to efficiently label tracking datasets comprehensively. In this work, we introduce SPAM, a video label engine that provides high-quality labels with minimal human intervention. SPAM is built around two key insights: i) most tracking scenarios can be easily resolved. To take advantage of this, we utilize a pre-trained model to generate high-quality pseudo-labels, reserving human involvement for a smaller subset of more difficult instances; ii) handling the spatiotemporal dependencies of track annotations across time can be elegantly and efficiently formulated through graphs. Therefore, we use a unified graph formulation to address the annotation of both detections and identity association for tracks across time. Based on these insights, SPAM produces high-quality annotations with a fraction of ground truth labeling cost. We demonstrate that trackers trained on SPAM labels achieve comparable performance to those trained on human annotations while requiring only $3-20\%$ of the human labeling effort. Hence, SPAM paves the way towards highly efficient labeling of large-scale tracking datasets. We release all models and code.

==> tables/ablation_labelquality.tex <==
%!TEX root = ../main.tex
\begin{table}[tb]
\center
\tabcolsep=0.11cm

    \resizebox{\columnwidth}{!}{
    \begin{tabular}{l | l | l | c c c}
     \toprule
     Row & Node & Edge & HOTA $\uparrow$& MOTA $\uparrow$ & IDF1 $\uparrow$  \\ [0.5ex] 
     \midrule
     1 & \xmark & \xmark & 65.1 & 69.4 & 80.6  \\
     \midrule
     2& Random & Random & 65.6 & 69.9 & 81.4  \\
     3&Img. Entropy & Random & 65.8 & 70.1 & 81.7 \\
     4&Box Entropy & Random & 65.8 & 70.7 & 81.5 \\
     5&Box Entropy & Uniform & -- & -- & -- \\
     6&Box Entropy & Ours & 67.1 & 73.4 & 83.2 \\
     7&Coreset~\cite{coreset} & Ours & 67.3 & 73.3 & 83.6 \\
     8&Ensemble~\cite{ensemble} & Ours & 67.4 & 73.0 & 83.7 \\
     9&Consistency~\cite{al_ili} & Ours & 67.1 & 73.7 & 83.2 \\
     \midrule
     10& \multicolumn{2}{|c|}{Ours} & 71.0 & 81.5 & 89.0  \\
     \midrule 
     11& \multicolumn{2}{|c|}{Oracle} & 74.1 & 88.9 & 93.2 \\
    \midrule


\end{tabular}}

\caption{Comparison label quality with baselines for association and AL for object det literature with 4000 annotations (1\% of annotation effort). \TODO{We could also create an additional line graph with different ratios of annotation effort on top of this table}\TODO{description}}

\label{table:quality}
\end{table}

